Impact of Property Covariance on Cluster Weak lensing Scaling Relations

We present an investigation into a hitherto unexplored systematic that affects the accuracy of galaxy cluster mass estimates with weak gravitational lensing. Specifically, we study the covariance between the weak lensing signal, $\Delta\Sigma$, and the "true" cluster galaxy number count, $N_{\rm gal}$, as measured within a spherical volume that is void of projection effects. By quantifying the impact of this covariance on mass calibration, this work reveals a significant source of systematic uncertainty. Using the MDPL2 simulation with galaxies traced by the SAGE semi-analytic model, we measure the intrinsic property covariance between these observables within the 3D vicinity of the cluster, spanning a range of dynamical mass and redshift values relevant for optical cluster surveys. Our results reveal a negative covariance at small radial scales ($R \lesssim R_{\rm 200c}$) and a null covariance at large scales ($R \gtrsim R_{\rm 200c}$) across most mass and redshift bins. We also find that this covariance results in a $2-3\%$ bias in the halo mass estimates in most bins. Furthermore, by modeling $N_{\rm gal}$ and $\Delta\Sigma$ as multi-(log)-linear equations of secondary halo properties, we provide a quantitative explanation for the physical origin of the negative covariance at small scales. Specifically, we demonstrate that the $N_{\rm gal}$-$\Delta\Sigma$ covariance can be explained by the secondary properties of halos that probe their formation history. We attribute the difference between our results and the positive bias seen in other works with (mock)-cluster finders to projection effects. These findings highlight the importance of accounting for the covariance between observables in cluster mass estimation, which is crucial for obtaining accurate constraints on cosmological parameters.

==> app_old.tex <==

\section{Particle Resolution and its impact on measurement errors} 
\label{sec:ptcl_resolution}
With the 300 Cori Haswell node hours allocated by the NERSC to this project, we were able to make measurements of $\Delta\Sigma$ for $\sim 5000$ clusters using dark matter particles downsampled by a factor of 10, in 20 log-spaced radial bins, at a projection depth of $200~h^{-1}\rm Mpc$. 

At a downsampling rate of 10, our effective dark matter particle resolution is $M_{\rm p} \approx 1.51 \times 10^{10} h^{-1}M_\odot$. The error in $\Delta\Sigma$ comes from three sources: (i) cosmic variance, (ii) Poisson noise, and (iii) the intrinsic diversity of halos accounted for by secondary halo properties. In \S\ref{subsec: DS_Xparam}, we presented the contribution to $\Delta\Sigma$ scatter from secondary halo properties. Here, we compare the Poisson noise to the cosmic variance floor. 

The cosmic variance introduces fluctuations in a 2D surface density fluctuation, given by 
\beqa
\delta\Delta\Sigma(R) = D_p \rho_m \sigma(R),
\label{eqn:cosmic_2d_density_fluctuation}
\eeqa
where $D_{p} = 200 h^{-1}\rm Mpc$ is the projection depth, $\rho_m(z)$ is the mean density of the universe at that redshift, and $\sigma(R)$ is the root mean squared matter density fluctuation, given by 
\beqa
\sigma^2(R) = \int\Delta^2(k)\Big(\frac{3j_1(kR)}{kR}\Big)^2 d\ln{k},
\label{eqn:cosmic_variance}
\eeqa
which is smoothed over an area of $A=4\pi R^2$, $\Delta^2(k)$ is the matter power spectrum for a wavenumber $k$, and $j_1$ is the Bessel function of the first order. 

Figure~\ref{fig:ptcl_resolution} shows the standard error of $\Delta\Sigma$ at a benchmark bin $M_{\rm 200c} \in [1\times10^{14}, 2\times10^{14}) M_{\odot}h^{-1}$ at z=0.00. At particle downsampling factors of 200, 100, and 10, the reduction in error is consistent with the Poisson term of $\sqrt{N}$, indicating that at these sampling rates, Poisson noise dominates. At our current downsampling rate of nth=10, the standard error is just above the cosmic variance floor at small scales and drops below the cosmic variance floor at large scales. In the ideal case that Poisson noise accounts for all the standard error, fully sampling all particles (nth=1, red dotted line) will reduce the standard error by a factor of $\sqrt{10}$, rendering it just below the cosmic variance floor at small scales. In the realistic case that the standard error for $\Delta\Sigma$ contributes from both Poisson noise and the intrinsic diversity of halo profiles, the fully sampled standard error should be on par with the cosmic variance at small scales. A future study with fully sampled particles should yield greater statistical constraints. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{plots/ptcl_resolution_error.pdf}
    \caption{The standard error of $\Delta\Sigma$ measurements tested on a benchmark bin of $M_{\rm 200c} \in [1\times10^{14}, 2\times10^{14}) M_{\odot}h^{-1}$ at z=0. The standard error is estimated using the bootstrap method for the $N=500$ clusters with dark matter particles downsampled by a factor of 200, 100, and 10 (solid lines). At our current resolution (nth=10, solid green line), the standard error is just above the cosmic variance at small scales and drops below the cosmic variance at large scales. The solid black line is density fluctuation estimated from the cosmic variance floor, as described in Equations~\eqref{eqn:cosmic_variance} and \eqref{eqn:cosmic_2d_density_fluctuation}. In the ideal case that Poisson noise accounts for all the standard error, fully sampling all particles ($n{\rm th}=1$, red dotted line) will reduce the standard error by a factor of $\sqrt{10}$, rendering it just below the cosmic variance floor at small scales. In the realistic case that the standard error for $\Delta\Sigma$ contributes from both Poisson noise and the intrinsic diversity of halo profiles, the fully sampled standard error should be on par with the cosmic variance at small scales.}
    \label{fig:ptcl_resolution}
\end{figure}


\section{Robustness testing of Covariance Modeling}
\label{sec:cov_robustness}
The shape posterior is sampled by a Monto Carlo Markov Chain (MCMC) using the ecmee package \citep{Foreman_Mackey_2013}. We test for convergence by ensuring that the number of steps exceeds $t_{\rm auto}/100$ for all parameters, where $t_{\rm auto}$ is the integrated autocorrelation time as defined by \citet{Goodman_Weare_2010} and by ensuring that the convergence diagnostic denoted with $R$ \citep{Gelman_Rubin_92} across all walkers satisfy $R < 1.05$. 

The posterior distribution according to Bayes theorem is given as:
\begin{align}
    p(\boldsymbol{\theta}|\{y_{i}\}) &\propto p({\{y_{i}\}|\boldsymbol{\theta}})p({\boldsymbol{\theta}}) \\
    &= \prod_{i} p({y_{i}|\boldsymbol{\theta}})p({\boldsymbol{\theta}}),
\end{align}
where the second line assumes independent and identical distribution ($\mathrm{i.i.d}$) for the data vectors. We set uniform priors $p({\boldsymbol{\theta}})$ shown in Table ~\ref{tab:prior} with signs and ranges motivated by the shape of the covariance (i.e., a negative $\gamma$ and positive $\tau$ to offset $f(\tilde{x})$ to the left and a positive $s$ and negative $g$ shifts the fitted curve downwards). 

We measure the goodness of fit using the left-tail $p$-value for the $\chi^2$ with $N_{\rm data} - N_{\rm dim} = 20 - 4 = 16$ degrees of freedom. We compare between models by the Deviance Information Criterion defined as
\begin{equation}
    \mathrm{DIC} = 2\overline{ D(\boldsymbol{\theta})} - D(\boldsymbol{\overline{\theta}}),
\end{equation}
where $\overline{\theta}$ is the best-fit parameters, and $D(\boldsymbol{\theta})$ is defined as
\begin{equation}
    D(\boldsymbol{\theta}) \equiv -2\log{(P({\{x_{i}\}|\boldsymbol{\theta}}))}.
\end{equation}
The performance between different functional forms (Table \ref{tab:cov_functional_form}) is reported in Table~\ref{tab:prior}.

The summary statistics for the posterior distribution of the covariance models are listed in Table~\ref{tab:cov_best_fit_param_full_model} as plotted against measurements in Figure~\ref{fig:cov_function_compare}. Among the functions, the error function has either a better or comparable fit to all other functions in all other bins, as indicated by their DIC parameters. In two bins $M_{\rm 200c} \in [5\times10^{14},1\times10^{15})$ at $z=0.49$ and $M_{\rm 200c} \in [2\times10^{14},5\times10^{15})$ at $z=1.03$, the amplitude of the covariance is too small relative to their errors for shape parameters to be well-constrained. The right tail $p$-value for $\chi^2$ is $p > 0.05$ for all but one bin. For this reason, we take the full error function as the nominal functional form. 

For $R \geq R_{\rm vir}$ or $R \geq R_{\rm 200c}$, we find the covariance to be null at $p$-values $> 0.01$. Assuming that the covariance is 0 at large scales, we can set $g=-1$ where we have the reduced model. We compare the results of the error function of the reduced model to the full model and find their performance varies from bin to bin as indicated by the DIC (Table \ref{tab:error_func_reduced}). The posteriors of the reduced model provide marginally tighter constraints than the full model (Figure \ref{fig:cov_cornerplot}). 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{plots/cov_M200c_Dsep_R200c_all_models.pdf}
    \caption{Comparison of Cov($\Delta\Sigma$, $N_{\rm gal}$) and different functional forms using the full model. The functions are classes of "Sigmoid" functions. In all bins, the error function outperforms other functional forms in their DIC parameters providing good $\chi^2$ values. For $M_{\rm 200c} \in [5\times10^{14},1\times10^{15})$ at $z=0.49$ and $M_{\rm 200c} \in [2\times10^{14},5\times10^{15})$ at $z=1.03$, the posteriors for the full models do not converge as the size of the covariance is too small.}
    \label{fig:cov_function_compare}
\end{figure*}


\begin{table*}
\centering
\ra{1.3}
    \begin{tabular}{lllllllll} \toprule
    \multirow{2}{*}{Mass \& redshift} & \multicolumn{8}{c}{Error function (full): $s\Big( {\rm erf}(\frac{\sqrt{\pi}}{2} \tilde{x}) + g\Big)$} \\
    \cmidrule{2-9}
    & $\tau$ & $\gamma$  & $g$ & $10^{12}\times s$ & $\Delta \rm DIC_{\rm log}$ & $\Delta \rm DIC_{\rm alg}$ & $\Delta \rm DIC_{\rm arctan}$ & $p$-value  \\ \midrule
    %z=0.00
    $[5\times10^{13},1 \times 10^{14})$, $z=0.00$ & $0.47^{0.06}_{0.05}$ & $-0.66^{0.08}_{0.11}$ & $-0.99^{0.005}_{0.004}$ & $2.88^{0.71}_{0.47}$ & 4.8 & 17.8 & 31.5 & 0.27 \\
    $[1\times10^{14},2\times10^{14})$, $z=0.00$ & $0.57^{0.11}_{0.08}$ & $-0.76^{0.14}_{0.22}$ & $-1.008^{0.0005}_{0.0007}$ & $2.73^{0.13}_{-0.65}$ & -2.9 & -1.7 & 2.8 & 0.88 \\
    $[2\times10^{14},5\times10^{14})$, $z=0.00$ & $0.41^{0.04}_{0.04}$ & $-0.51^{0.05}_{0.06}$ & $-0.997^{0.004}_{0.0004}$ & $1.93^{0.24}_{0.18}$ & 4.4 & 17.4 & 35.0 & 0.79 \\
    $[5\times10^{14},1\times10^{15})$, $z=0.00$ & $0.27^{0.03}_{0.03}$ & $-0.40^{0.04}_{0.05}$ & $-1.006^{0.005}_{0.0005}$ & $1.03^{0.13}_{0.11}$ & -0.27 & 14.3 & 29.1 & 0.0009 \\
    \hline
    %z=0.49
    $[5\times10^{13},1\times10^{14})$, $z=0.49$ & $0.28^{0.6}_{0.05}$ & $-0.36^{0.05}_{0.07}$ & $-0.990^{0.013}_{0.013}$ & $0.75^{0.11}_{0.09}$ & 2.7 & 9.0 & 15.1 & 0.72 \\
    $[1\times10^{14},2\times10^{14})$, $z=0.49$ &  $0.35^{0.07}_{0.06}$ & $-0.43^{0.07}_{0.09}$ & $-1.022^{0.016}_{0.017}$ & $0.81^{0.15}_{0.10}$ & 1.7 & 5.4 & 9.3 & 0.97 \\
    $[2\times10^{14},5\times10^{14})$, $z=0.49$ & $0.24^{0.08}_{0.07}$ & $-0.49^{0.07}_{0.10}$ & $-0.995^{0.012}_{0.011}$ & $0.51^{0.14}_{0.01}$ & 0.6 & 2.4 & 4.0 & 0.63 \\
    $[5\times10^{14},1\times10^{15})$, $z=0.49$ & \multicolumn{7}{c}{NA} \\
    \hline
    %z=1.03
    $[5\times10^{13},1\times10^{14})$, $z=1.03$ & $0.17^{0.05}_{0.04}$ & $-0.31^{0.05}_{0.05}$ & $-1.019^{0.020}_{0.022}$ & $0.35^{0.06}_{0.05}$ & 4.3 & 6.5 & 8.3 & 0.05 \\
    $[1\times10^{14},2\times10^{14})$, $z=1.03$ & $0.21^{0.06}_{0.05}$ & $-0.42^{0.05}_{0.06}$ & $-1.024^{0.013}_{0.0014}$ & $0.51^{0.09}_{0.07}$ & -0.3 & 3.3 & 6.1 & 0.01 \\
    $[2\times10^{14},5\times10^{14})$, $z=1.03$ & \multicolumn{7}{c}{NA} \\
    
    \bottomrule
    \end{tabular}
\caption{Summary statistics for Cov($\Delta\Sigma$, $N_{\rm gal} \mid M, z$) binned by $R_{\rm 200c}$ and $M_{200c}$, with $N_{\rm gal}$ defined inside the halo $R_{\rm 200c}$. Columns 2-5 are the best-fit parameters for the nominal error function and their $1\sigma$ ranges. Columns 6-8 are the difference between the DIC of the logistics, algebraic, and inverse tangent models with the nominal error function, respectively. Column 9 is the right-tail p-value as measured by the $\chi^2$ statistic with 20-4 = 16 degrees of freedom. Across all bins with applicable posterior constraints, the error function out-performs or is comparable to alternative functional forms as indicated by the difference in DIC, and has $p \geq 0.01$ in all but one bin. In two bins $M_{\rm 200c} \in [5\times10^{14},1\times10^{15})$ at $z=0.49$ and $M_{\rm 200c} \in [2\times10^{14},5\times10^{15})$ at $z=1.03$ the size of the covariance is too small relative to the size of their errors for shape parameters to be constrained. The covariance in these two bins is consistent with null at $p =0.01$ and $p=0.05$ levels, respectively.
}
\label{tab:cov_best_fit_param_full_model}
\end{table*}

\begin{table*}
\centering
\ra{1.3}
    \begin{tabular}{cccccc} \toprule
    \multirow{2}{*}{Mass \& redshift} & \multicolumn{5}{c}{Error function (reduced): $s\Big( {\rm erf}(\frac{\sqrt{\pi}}{2} \tilde{x}) -1 \Big)$} \\
    \cmidrule{2-6}
    & $\tau$ & $\gamma$  & $10^{12}\times s$ & $\Delta \rm DIC_{\rm erf-full}$  & p-value  \\ \midrule
    %z=0.00
    $[5\times10^{13},1 \times 10^{14})$, $z=0.00$ & $0.44^{0.04}_{0.04}$ & $-0.63^{0.07}_{0.09}$  & $2.66^{0.56}_{0.39}$ & -5.2 & 0.06 \\
    $[1\times10^{14},2\times10^{14})$, $z=0.00$ & $0.69^{0.11}_{0.09}$ & $-0.98^{0.20}_{0.27}$  & $4.10^{2.31}_{1.19}$ & 4.5 & 0.96 \\
    $[2\times10^{14},5\times10^{14})$, $z=0.00$ & $0.40^{0.04}_{0.03}$ & $-0.50^{0.05}_{0.06}$  & $1.90^{0.26}_{0.20}$ & 0.2 & 0.78 \\
    $[5\times10^{14},1\times10^{15})$, $z=0.00$ & $0.29^{0.04}_{0.04}$ & $-0.40^{0.04}_{0.04}$  & $1.12^{0.13}_{0.11}$ & 6.1 & 0.005 \\
    \hline
    %z=0.49
    $[5\times10^{13},1\times10^{14})$, $z=0.49$ & $0.25^{0.04}_{0.03}$ & $-0.35^{0.04}_{0.04}$  & $0.79^{0.08}_{0.07}$ & 6.2 & 0.57 \\
    $[1\times10^{14},2\times10^{14})$, $z=0.49$ & $0.38^{0.14}_{0.09}$ & $-0.48^{0.12}_{0.24}$  & $0.85^{0.46}_{0.19}$ & -6.9 & 0.81 \\
    $[2\times10^{14},5\times10^{14})$, $z=0.49$ & $0.25^{0.21}_{0.12}$ & $-0.55^{0.14}_{0.42}$  & $0.40^{0.69}_{0.13}$ & NA & 0.48 \\
    $[5\times10^{14},1\times10^{15})$, $z=0.49$ & $0.61^{0.27}_{0.24}$ & $-0.90^{0.49}_{0.76}$  & $1.01^{3.05}_{0.60}$ & -5.7 & 0.99 \\
    \hline
    %z=1.03
    $[5\times10^{13},1\times10^{14})$, $z=1.03$ & $0.20^{0.06}_{0.05}$ & $-0.35^{0.06}_{0.08}$  & $0.38^{0.07}_{0.06}$ & -0.75 & 0.04 \\
    $[1\times10^{14},2\times10^{14})$, $z=1.03$ & $0.22^{0.06}_{0.05}$ & $-0.42^{0.06}_{0.8}$  & $0.54^{0.11}_{0.09}$ & 3.9 & 0.3 \\
    $[2\times10^{14},5\times10^{14})$, $z=1.03$ & $5.97^{2.76}_{3.01}$ & $-0.55^{3.30}_{2.99}$  & $0.02^{0.02}_{0.008}$ & NA & 0.15 \\
    
    \bottomrule
    \end{tabular}
\caption{Summary statistics for Cov($\Delta\Sigma, N_{\rm gal} \mid M, z$) binned by $R_{\rm 200c}$ and $M_{200c}$ with $N_{\rm gal}$ defined inside the halo $R_{\rm 200c}$ for the reduced error function model. Compared with the full error function model, the performance of the reduced model varies from bin to bin -- using $\Delta{\rm DIC} > 3$ as a statistically significant result, it outperforms the full model in 5/9 overlapping bins, under-performs in 3/9 bins, and is comparable in 2 bins. The reduced model is able to yield convergent chains for $M_{\rm 200c} \in [5\times10^{14},1\times10^{15})$ at $z=0.49$ and $M_{\rm 200c} \in [2\times10^{14},5\times10^{15})$ at $z=1.03$ but with poor constraints on the parameters. }
\label{tab:error_func_reduced}
\end{table*}

%%% Complete this table
\begin{table*}
\centering
\ra{1.3}
    \begin{tabular}{lcccccccccccc} \toprule
    \multirow{2}{*}{Redshift} & \multirow{2}{*}{R$^2$} &  \multirow{2}{*}{Const} & \multicolumn{2}{c}{$c_{\rm vir}$} & \multicolumn{2}{c}{T/|U|}  & \multicolumn{2}{c}{$a_{1/2}$} & \multicolumn{2}{c}{$\Gamma^*_{\rm 2dyn}$}  & \multicolumn{2}{c}{$X_{\rm off}$} \\
    \cmidrule{4-13}
    \& $M_{\rm 200c}$ ($M_{\odot}h^{-1}$) &  & & $\beta_{\Ngal}$ & $F$ & $\beta_{\Ngal,}$ & $F$ & $\beta_{\Ngal}$ & $F$ &
    $10^6\times \beta_{\Ngal}$ & $F$ & $10^3\times\beta_{\Ngal}$ & $F$ 

    \\ \midrule
    %z=0.00
    $z=0.00$  &&&&&&&&&&&& \\
    \multirow[t]{2}{*}{$[5\times10^{13}, 1\times10^{14})$} & .45 & -.69 & -.035(.004) & 171 & 1.448(.135) & 185 & .103(.084) & 166 & 2.743(1.68) & 134 & -2.(.XX) & 69  \\
    
    \multirow[t]{2}{*}{$[1\times10^{14}, 2\times10^{14})$} & .48 & -.46 & -.033(.003) & 217 & 1.086(.120) & 179 & -.198(.071) & 170 & 2.668(.628) & 206 & -1.(.XX) & 86  \\
        
    \multirow[t]{2}{*}{$[2\times10^{14}, 5\times10^{14})$} & .49 & -.41 & -.029(.003) & 196 & -.794(.086) & 145 & .292(.007) & 213 & -.722(.223) & 167 & .6(0.07) & 67  \\
        
    \multirow[t]{2}{*}{$[5\times10^{14}, 1\times10^{15})$} & .46 & -.32 & -.019(0.002) & 119 & 1.503(.068) & 111 & .148(.054) & 201 & .483(.096) & 226 & -.3(0.04) & 51  \\
    \hline
    
    %z=0.49
    $z=0.49$  &&&&&&&&&&&& \\
    \multirow[t]{2}{*}{$[5\times10^{13}, 1\times10^{14})$} &.25& -.71 & .006(.005) & 24 & .325(.125) & 69 & .188(.101) & 142 & 3.90(1.64) & 102 & -.3(.XX) & 35  \\
    
    \multirow[t]{2}{*}{$[1\times10^{14}, 2\times10^{14})$} & .21 & -.45 & -.450(.082) & 27 & .314(.135) & 46 & -.353(.158) & 107 & 1.80(.71) & 89 & -.5(.XX) & 14  \\
       
    \multirow[t]{2}{*}{$[2\times10^{14}, 5\times10^{14})$} & .13 & -.56 & -.003(.004) & 0 & .323(.110) & 26 & .670(.155) & 51 & .388(.108) & 26 & -.4(.XX) & 2  \\
       
    \multirow[t]{2}{*}{$[5\times10^{14}, 1\times10^{15})$} & .13 & -.32 & -.010(.008) & 0 & .007(.286) & 0 & .697(.309) & 5 & .-538(.331) & 3 & -.4(.XX) & 3  \\
    \hline
    
    %z=1.03
    $z=1.03$  &&&&&&&&&&&& \\
    \multirow[t]{2}{*}{$[5\times10^{13}, 1\times10^{14})$} & .27 & -1.12 & .015(.005) & 6 & .471(.136) & 21 & .569(.269)& 116 & 2.7(1.2) & 63 & -.9(.XX) & 0  \\
    
    \multirow[t]{2}{*}{$[1\times10^{14}, 2\times10^{14})$} & .22 & -.84 & .016(.004) & 10 & .374(.135) & 36 & -.233(.234) & 83 & 1.076(.478) & 36 & -.4(.XX) & 2  \\
        
    \multirow[t]{2}{*}{$[2\times10^{14}, 5\times10^{14})$} & .20 & -.6 & .0015(.005) & 10 & .284(.185) & 1 &  -.157(.266) & 15 & .160(.213) & 6 & -.6(.XX)
    & 13  \\
        
    \bottomrule
    \end{tabular}
\caption{The best-fit parameters and global $R^2$ for log-richness modeled in Equation~\eqref{eqn:model_richness_Xparam}. Quotes in parenthesis are the $1-\sigma$ error to the partial slope $\beta$. The partial F-statistic is used heuristically to quantify the explanatory power of each variable. Defined in Equation~\ref{eqn:F_partial}, the ratio between which is proportional to the $R^2$ that can be \textit{uniquely} explained by each variable alone. \dn{please update the values for Xoff, including non-zero errors.} } 
\label{tab:richness_multilinear_coeff}
\end{table*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{plots/GTC_models_M2e14_5e14_z0p00.pdf}
    \caption{Posterior distribution of shape parameters in a benchmark bin of $M_{\rm 200c}/M_{\rm vir} \in [2\times10^{14},5\times10^{14})$, $z=0.00$ under different binning schemes $r_p$ and $N_{\rm gal}$ models with different halo boundaries $R_{\rm halo}$. The marginalized parameter constraints for the full model closely overlap one another, and using the reduced model with $g=-1$ marginally improves the posterior constraints.}
    \label{fig:cov_cornerplot}
\end{figure*}

\section{Modeling Secondary Properties}
\label{sec:multilinear_modeling}

We describe the linear regression model for richness used in \S\ref{subsec:richness_Xparam}. The same methodology is applied to $\Delta\Sigma$ in \S\ref{subsec: DS_Xparam}. 

To model the expected natural logarithm of galaxy count ($\ln\Ngal$), we decompose it linearly using secondary halo parameters listed in Table~\ref{tab:notation_Xparam}, as shown in Equation~\eqref{eqn:model_richness_Xparam}. 
%We begin with a comprehensive list of secondary halo parameters from Table \ref{tab:notation_Xparam}, and 
We employ the least squares method for linear regression and examine redundancies in the parameters. For over half of the bins, the parameters $\Gamma_{\rm inst}$, $\Gamma_{\rm 100Myr}^$, $\Gamma_{\rm 2dyn}^$, and $\Gamma_{\rm peak}$ exhibit collinearity, with Variance Inflation Factors (VIF) exceeding 5. This outcome is expected, as these quantities represent the same physical quantities smoothed over different time scales. To determine which parameters to retain, we utilize the partial F-statistic.

We consider the partial F-statistic serves as a heuristic measure for the explanatory power of a variable, defined as:
\beqa
F_{\rm partial} = \frac{({\rm RSSE_{\rm reduced} - RSSE_{\rm full}})/p}{{\rm RSSE_{\rm full}}/(n-k)},
\label{eqn:F_partial}
\eeqa
where RSSE is the residual sum of squared errors for the reduced model after removing the parameter in question and the full model containing $\Pi \in$~\{$a_{1/2}$, $c_{\rm vir}$, $T/U$, $\Gamma_{\rm 2dyn}^*$, $X_{\rm off}$\}, $p$ is the number of parameters removed from the full model which in our case is by construction set to $p = 1$, $n$ the number of data points, and $k$ is the number of parameters in the full backward model. From this statistic, it can be shown to be proportional to the contribution to the total $R^2$ \textit{uniquely} explained by this parameter alone.  

A partial F-statistic test shows that $\Gamma_{\rm 2dyn}^*$ has the highest partial F-statistic, so this is the parameter we preserve in the reduced dimensional linear regression. In our final model we are left with the parameters \{$a_{1/2}$, $c_{\rm vir}$, $T/U$, $\Gamma_{\rm 2dyn}^*$, $X_{\rm off}$\}. We apply the following tests to check for the robustness of the linear model in all bins:
\begin{itemize}
    \item Variance inflation factor (VIF) test with a cutout of 5 to check for multicollinearity,
    \item Global F-statistic for the entire model at a p-value of 0.05 to check for correlation of dependent-variable with respect to all parameters.
    \item Partial F-statistic for the entire parameter to compare the relative importance of each parameter. The Partial F-statistic is proportional to the $R^2$ that each additional parameter uniquely adds to the multi-linear fit. 
    \item T-statistic for each parameter to check that the coefficients are not consistent with 0 at a p-value of 0.05.
    \item Breusch-Pagan Lagrange Multiplier test \citep{Breusch_Pagan_1979} for heteroscedasticity at a p-value of 0.05.
    \item Shapiro-Wilk test \citep{Shapiro_Wilk_1965} for Gaussianity of residuals at a p-value of 0.05.
\end{itemize}
In all bins, the reduced model passes the first four tests. In some bins, they fail the Shapiro-Wilk test due to a negative skew and positive kurtosis, but a visual examination from Q-Q\dn{What is Q-Q plots?} plots shows that the residuals are mostly Gaussian except at the tail ends. 

\section{Testing for Gaussianity of $P(\DSig, \ln\Ngal \mid M,z)$} \label{subsec:Cov_test_normal}

The joint distribution can be decomposed into
\beq
    P(\Delta\Sigma, \ln\Ngal \mid M,z) = P(\Delta\Sigma \mid \Ngal, M, z) P(\ln\Ngal \mid M,z).
    \label{eq:Bayes_P_DS_lambda}
\eeq
We assume that (a) $P(\ln\Ngal | M, z)$ can be described with a normal distribution \citep[e.g.,][]{Costanzi_2021, cluster_cosmo2021DES, To_2021} and (b) $P(\Delta\Sigma, \ln\Ngal \mid M,z)$ follows a bivariate normal distribution. Then, it follows that $P(\Delta\Sigma \mid \Ngal, M, z)$ follows a normal distribution with mean relation:
\beq
    \avg{\Delta\Sigma \mid \Ngal, M, z} = \avg{\Delta\Sigma \mid M, z}
    + r\sigma_{\DS} \frac{\ln\Ngal - \avg{\ln\Ngal \mid M, z}}{\sigma_{\Ngal}}.
\label{eq:mean_obs_given_m}
\eeq

We derive the coefficients in Equation~\eqref{eq:mean_obs_given_m} by modeling richness as a linear function of halo parameters in Equation~\eqref{eqn:model_richness_Xparam}. We prove this assertion in Appendix~\ref{sec:proof_DS_given_lambda} and show that the $P(\Delta\Sigma \mid \Ngal, M, z)$ has mean relation
\begin{align}
    \label{eq:DS_given_lambda_Xparam_mean}
    \avg{\Delta\Sigma | \Ngal, M, z } ~=&~ \avg{\ln{\Delta\Sigma}|N_{\rm gal}}_0 \\ \nonumber 
        +& C_1\sigma_{\DS}\Big(\sum_i{\frac{\beta_{\Ngal,i} }{\sigma_{\Pi_i}}\rho_{\Delta\Sigma-\Pi_i}\times}(\Pi_i - \avg{\Pi_i | m, z})\Big),
\end{align}
and Gaussian scatter with variance
\begin{align}
\label{eq:DS_given_lambda_Xparam_var}
\qquad \sigma^2_{\DS|\Ngal} \quad =&~  \sigma^2_{0} +  C_2\sum_i{\beta_{\Ngal,i}^2 \sigma^2_{\Pi_i}(1-\rho^2_{\Delta\Sigma-\Pi_i})} \\ \nonumber
&\ \ + C_3\sum^{j\neq i}_{i,j}{\rho_{\Pi_i-\Pi_j}\sigma_{\Pi_i}\sigma_{\Pi_j}}.
\end{align}

Hence, we can test the bivariate assumption of $P(\Delta\Sigma, \ln\Ngal \mid M,z)$ by testing if $P(\Delta\Sigma \mid \Ngal, M, z)$ can be described as a multi-linear model of secondary halo parameters using our linear-regression machinery developed in Appendix \ref{sec:multilinear_modeling}. In Section \ref{subsec: DS_Xparam} we demonstrated that this is the case, and therefore $P(\Delta\Sigma, \ln\Ngal \mid M,z)$ can be modeled as a bivariate distribution with its full shape information captured by $\text{Cov}(\Delta\Sigma, \ln\Ngal)$.

% Conversely, the normality of $P(\Delta\Sigma | \Ngal, M, z)$ with a mean given by a linear combination of secondary halo parameters $\vec{\Pi_i}$ equates to $P(\Delta\Sigma, \ln\Ngal | M, z) \propto \mathcal{N}$, as shown in Equation~\eqref{eq:Bayes_P_DS_lambda}. Armed with the machinery for multi-linear regression developed in \S\ref{sec:Xparams_cov}, we can test the validity of describing the correlation between $\Delta\Sigma$ and $\ln\Ngal$ entirely by their covariance matrix. \arya{This is already explained above, no need for repetition. }

\section{Derivation of $P(\Delta\Sigma \mid \Ngal, m, z)$}
We demonstrate that $P(\Delta\Sigma \mid \Ngal, M, z)$ can be modeled as a multi-linear relation of secondary halo parameters. As discussed in Appendix \ref{subsec:Cov_test_normal} this is needed to show that $P(\Delta\Sigma, \Ngal \mid M, z)$ is a bivariate distribution with its full shape information captured by $\text{Cov}(\Delta\Sigma, \ln\Ngal \mid M, z)$.

\label{sec:proof_DS_given_lambda}
From our assertion that $P(\Delta\Sigma, \vec{\Pi} \mid M, z)$ is a bivariate normal, the conditional probability $P(\Pi_i \mid \Delta\Sigma, M, z)$ in each radial bin can be expressed as a normal distribution with mean
\beq
\avg{\Pi_i|\Delta\Sigma,  M, z} = \avg{\Pi_i | M, z}+ \rho_{\Pi_i-\Delta\Sigma}\frac{\sigma_{\Pi_i}}{\sigma_{\Delta\Sigma}} (\Delta\Sigma - \avg{\Delta\Sigma | M, z}),
\label{eq:Pi_given_DS_mean}
\eeq
and variance
\beq
\sigma_{\Pi_i | \Delta\Sigma}^2 = \sigma^2_{\Pi_i}(1-\rho^2_{\Pi_i-\Delta\Sigma}). 
\label{eq:Pi_given_DS_var}
\eeq
Here, we omit the radial dependence $R/R_{\rm 200c}$ for all variables and the conditional dependence on $(M, z)$ in the subscripts for $\rho$ and $\sigma$ (i.e., $\sigma_{\Delta\Sigma}$ should be explicitly written as $\sigma_{\Delta\Sigma| M, z}$). We expect the scatter $\sigma_{\Delta\Sigma}$ to vary in bins of $(M, z, r_p)$, \dn{the following sentences is hard to understand; rephrase.}but it remains constant in the bin under the homoscedasticity assumption for small enough bins. 

For an independent random variable $Z = X+Y$ with $X$ and $Y$ uncorrelated independent random variables with distributions of the form $\sim \mathcal{N}(u,\sigma^2)$ and $\sim \mathcal{N}(\nu,\tau^2)$, respectively, Z is another Gaussian of $\mathcal{N}(u+v, \sigma^2 + \tau^2)$. In the case that X and Y are correlated, we must introduce a cross term in the variance of probability distribution Z, namely $P(Z) \sim \mathcal{N}(u+v, \sigma^2 + 2\rho_{X-Y}\sigma\tau + \tau^2)$. 

In our specific case, we want to model the distribution $P(\sum_i \beta_{s,i}\Pi_i \mid \Delta\Sigma, M, z)$ from $P(\Pi_i \mid \Delta\Sigma, M, z)$ and the correlation here refers to the correction between secondary halo parameter $\rho_{\Pi_i, \Pi_j}$.\footnote{In \S\ref{subsec: DS_Xparam}, we show through the Variance Inflation test that set of reduced model parameters $\Pi \in \{a_{1/2}, c_{\rm vir}, T/U, \Gamma_{\rm 2dyn}^*, X_{\rm off} \}$ are not multi-collinear.} 
%However, as demonstrating multi-collinearity is a looser criterion than demonstrating non-correlation, we cannot assume the set of reduced secondary halo parameters are not correlated, and hence must take into account the correlated cross-term in computing the variance for the probability distribution of a weighted sum of these parameters. 
%Since these parameters are correlated, halos with high concentration form earlier, so they would have smaller values of $a_{1/2}$, the characteristic scale at which is main progenitor of the halo by following the halo merger tree is half the mass of the halo at the epoch in the snapshot; fully virialized (earlier forming) halos would also have smaller values of $T/|U|$, mass accretion rate $\Gamma_{\rm 2dyn}^*$ and $X_{\rm off}$. In the absence of occasional fly-by objects, high values of these parameters point to the ongoing gravitational collapse and infall of matter for clusters undergoing virialization. Quantitatively, \citet{Shin_2023} produced the correlation of such secondary halo parameters from results on a suite of N-body simulations.

From the convolution theorem and the expressions for $P(\Pi_i \mid \Delta\Sigma, M, z)$ in Equations~\eqref{eq:Pi_given_DS_mean} and \eqref{eq:Pi_given_DS_var}, we obtain the expression for $P(\ln\Ngal \mid \Delta\Sigma, M, z)$ as a normal distribution with mean:
\begin{align}
\avg{\ln\Ngal | \Delta\Sigma, M, z } ~=&~ \avg{\ln N_{\rm gal,0}|\Delta\Sigma, M, z}+ \\ \nonumber 
& \sigma_{\Delta\Sigma}\Big(\sum_i{\frac{\beta_{\Ngal,i}}{\sigma_{\Pi_i}}\rho_{\Delta\Sigma-\Pi_i}\times}(\Pi_i - \avg{\Pi_i | M, z})\Big),
\end{align}
and variance
\begin{align}
\qquad \sigma^2_{\ln{\Ngal}|\Delta\Sigma} \quad =&~  \sigma^2_{N_{\rm gal,0}} +  \sum_i \beta_{\Ngal,i}^2 \sigma^2_{\Pi_i}(1-\rho^2_{\Delta\Sigma-\Pi_i}) + \\ \nonumber
& \sum^{j\neq i}_{i,j}\rho_{\Pi_i-\Pi_j}\sigma_{\Pi_i}\sigma_{\Pi_j}.
\end{align}

Our goal is to show that $P(\Delta\Sigma | \Ngal, M, z)$ is normally distributed. From the Bayes theorem,
\beqa
P(\Delta\Sigma \mid \Ngal, M, z) = P(\ln\Ngal \mid \Delta\Sigma, M, z) \frac{P{(\Delta\Sigma \mid M, z)}}{P(\ln\Ngal \mid M, z)}.
\eeqa
Assuming once again that $P(\ln\Ngal | M, z)$ and $P(\Delta\Sigma | M, z)$ can be modeled as normal distributions, then  $P(\Delta\Sigma \mid \Ngal, M, z)$ is another normal distribution with mean 
\begin{align}
\label{eq:DS_given_lambda_Xparam_mean_append}
\avg{\Delta\Sigma | \Ngal, M, z } ~=&~ \avg{\Delta\Sigma|N_{\rm gal,0}, M, z} \\ \nonumber 
+& C_1\sigma_{\Delta\Sigma}\Big(\sum_i \frac{\beta_{\Ngal,i} }{\sigma_{\Pi_i}}\rho_{\Delta\Sigma-\Pi_i} \times (\Pi_i - \avg{\Pi_i | M, z})\Big)
\end{align}
and variance
\begin{align}
\label{eq:DS_given_lambda_Xparam_var_append}
\qquad \sigma^2_{\Delta\Sigma|\ln{\Ngal}} \quad =&~  \sigma^2_{0} +  C_2\sum_i{\beta_{\Ngal,i}^2 \sigma^2_{\Pi_i}(1-\rho^2_{\Delta\Sigma-\Pi_i})}+ \\ \nonumber
& C_3\sum^{j\neq i}_{i,j}{\rho_{\Pi_i-\Pi_j}\sigma_{\Pi_i}\sigma_{\Pi_j}}.
\end{align}
The parameters $C1$, $C2$, $C3$, and $\sigma_0$ can be explicitly derived if we know the posterior distribution of  $P(\ln\Ngal | M, z)$ and $P(\Delta\Sigma | M, z)$ by the exercise of completing the squares inside the exponents, but the exact values are not essential for this paper. 

\section{Modeling mass-dependence with KLLR}

Kernel local linear regression (KLLR) builds localized linear profiles around an independent variable which in our case are $\Delta\Sigma (M,z, r_p)$ and $\ln\Ngal-\ln M$ conditioned on the independent variable $\ln M$. The localized linear fits are fitted to minimize the weighted squared error around each pivot mass, given by
\beqa
\epsilon^2_i(M_0,z) = \sum^n_j w_j (s_{i,j} - \alpha_i(M,z)\ln{(M/M_0)} - \pi_i(M,z))^2,
\label{eqn:weighted_err}
\eeqa
where the weight $w_j$ of each data point is governed by a Gaussian kernel of the form
\beqa
w_j = \frac{1}{\sqrt{2\pi\sigma_{\rm LLR}^2}}\exp{\biggl\{-\frac{\ln{(M/M_0)}^2}{2\sigma^2_{\rm LLR}} \biggr\} },
\label{eq:Gaussian_kernel_KLLR}
\eeqa
$\alpha_i$ and $\pi_i$ are the slope and intercept for the mean relations (Equations~\ref{eq:model_richness} and \ref{eq:model_wl}) around a pivot mass $M_0$, $i \in \{\Delta\Sigma, \ln \Ngal\}$, and the total error squared summed over all data points $j$.

We find that the local slope $\alpha_i$, intercept $\pi_i$, and scatter $\sigma_{i|M}$ are insensitive to the kernel width $\sigma_{\rm LLR}$ so long as the kernel width times the number of pivot points for $\ln M$ cover the entire dynamic mass range. We choose enough pivot points to reduce the mass-dependent scatter but not too many to prevent overfitting. 

In our $\ln \Ngal-\ln M$ models governed by Equation~\ref{eq:model_richness} and shown in Figure~\ref{fig:MOR_DMPL2_vs_data}, we relax the assumption of global log-linearity and determine the local linear fit using KLLR. We apply 6 equally log-spaced bins in the mass range of $\log{M/M_{\odot}} \in [13.7,15)$ with a Gaussian kernel with the width of $\sigma_{\rm LLR} = 0.2$ dex.

In our localized $\Delta\Sigma (r_p)$ model for each radial bin, we fit Equation~\ref{eq:model_wl} using 10 equally log-spaced mass bins within each (M,z) bin. We choose the kernel width as $\sigma_{\rm LLR} = 0.1$ dex. 

Figure~\ref{fig:DS_KLLR} shows fits to $\Delta\Sigma(r_p)$ at three representative radial bins by KLLR and compares the localized scatter conditioned on the mass versus the global scatter. We find that applying KLLR reduces the size of the scatter by removing the mass dependency of the mean profiles.  

\label{sec:KLLR_robustness}
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=0.8\textwidth]{plots/mean_DS_KLLR_0.18.pdf}
     \end{subfigure}
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=0.8\textwidth]{plots/mean_DS_KLLR_0.45.pdf}
     \end{subfigure}
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=0.8\textwidth]{plots/mean_DS_KLLR_3.5.pdf}
     \end{subfigure}
        \caption{Fits to $\Delta\Sigma(r_p)$ at $r_p = R/R_{\rm 200c}$ of 0.18, 0.45 and 3.5 over the mass range of $\log{M_{\rm 200c}/M_{\odot}} \in [13.7,15)$. Black lines are the global mean profiles, and the blue lines are the localized mean profiles conditioned on mass as measured by the KLLR algorithm. KLLR reduces the scatter by removing the variance in $\Delta\Sigma$ caused by the change in halo mass.}
        \label{fig:DS_KLLR}
\end{figure}

